Bayesian Evidences for Dark Energy models in light of current obsevational data

We do a comprehensive study of the Bayesian evidences for a large number of dark energy models using a combination of latest cosmological data from SNIa, CMB, BAO, Strong lensing time delay, Growth measurements, measurements of Hubble parameter at different redshifts and measurements of angular diameter distance by Megamaser Cosmology Project . We consider a variety of scalar field models with different potentials as well as different parametrisations for the dark energy equation of state. Among 21 models that we consider in our study, we do not find strong evidences in favour of any evolving dark energy model compared to $\Lambda$CDM. For the evolving dark energy models, we show that purely non-phantom models have much better evidences compared to those models that allow both phantom and non-phantom behaviours. Canonical scalar field with exponential and tachyon field with square potential have highest evidences among all the models considered in this work. We also show that a combination of low redshift measurements decisively favours an accelerating $\Lambda$CDM model compared to a non-accelerating power law model.

==> tablefull.tex <==
\begin{table}[H]
\centering
%\resizebox{1\textwidth}{!}{\begin{minipage}{\textwidth}
\caption{Log Evidence($\mathcal{Z}$)}
\begin{tabular}{lccc}
\Xhline{2\arrayrulewidth}
\textbf{Model} & \begin{small}$SNIa+CMB$\end{small}& \begin{small}$SNIa+CMB$\end{small} & \begin{small}$SNIa+CMB$\end{small}\\
               & \begin{small}$BAO$\end{small}  & \begin{small}$BAO+GROWTH$\end{small} & \begin{small}$BAO+GROWTH$\end{small} \\
               &       &             &  \begin{small}$H(Z)$\end{small}\\
\Xhline{2\arrayrulewidth}
$\Lambda$CDM & -30.63$\pm$0.16 & -36.15$\pm$0.17 &-52.66$\pm$0.17\\
$w$CDM & -32.54$\pm$0.17 & -38.11$\pm$0.18 & -53.28$\pm$0.19\\
CPL & -33.43$\pm$.17	& -39.05$\pm$.19	& -53.87$\pm$.19\\
7CPL & -32.91$\pm$0.17 & -38.39$\pm$0.18 & -53.33$\pm$0.19\\
BA & -33.29$\pm$0.17  & -38.95$\pm$0.18 & -53.85$\pm$0.19\\
JBP & -32.95$\pm$0.17 & -38.41$\pm$0.18 & -53.56$\pm$0.19\\
Exponential Galileon (thaw) & -29.13$\pm$0.14 & -34.65$\pm$0.16 & -51.68$\pm$0.16\\
Exponential Scalar (thaw)	& -29.09$\pm$0.14 & -34.56$\pm$0.16 & -50.57$\pm$0.16\\
Exponential Tachyon (thaw)	& -29.32$\pm$0.15 & -34.56$\pm$0.16 & -50.81$\pm$0.16\\
Inverse Galileon (thaw)	& -29.08$\pm$0.14 & -34.68$\pm$0.16 & -51.58$\pm$0.16\\
Inverse Scalar (thaw)	&-28.89$\pm$0.14 & -34.36$\pm$0.16 & -50.66$\pm$0.16\\
Inverse Tachyon (thaw) & -29.07$\pm$0.15 & -34.94$\pm$0.16 & -50.96$\pm$0.16\\
Linear Galileon (thaw)	& -29.27$\pm$0.14 & -34.87$\pm$0.16 & -51.77$\pm$0.16\\
Linear Scalar (thaw)	& -28.97$\pm$0.14 & -34.62$\pm$0.16 & -50.52$\pm$0.16\\
Linear Tachyon (thaw) & -29.52$\pm$0.15 & -34.64$\pm$0.16 & -51.17$\pm$0.17\\
Square Galileon (thaw) & -29.32$\pm$0.15 & -34.73$\pm$0.16 & -51.59$\pm$0.16\\
Square Scalar (thaw) & -29.00$\pm$0.14 &-34.52$\pm$0.16 & -50.41$\pm$0.16\\
Square Tachyon (thaw) & -29.26$\pm$0.15 & -34.86$\pm$0.16 & -51.35$\pm$0.17\\
GCG track & -33.49$\pm$0.18 & -38.99$\pm$0.19 & -56.63$\pm$0.20\\
GCG thaw & -31.87$\pm$0.16 & -37.17$\pm$0.17 &-54.41$\pm$0.18\\
Scalar Tracker	& -30.96$\pm$0.16  & -36.79$\pm$0.17 & -54.12$\pm$0.18\\
\Xhline{2\arrayrulewidth} 
\end{tabular} 
 %\end{minipage}}
\end{table}

